On the computational and statistical complexity of over-parameterized matrix sensing

We consider solving the low rank matrix sensing problem with Factorized Gradient Descend (FGD) method when the true rank is unknown and over-specified, which we refer to as over-parameterized matrix sensing. If the ground truth signal $\mathbf{X}^* \in \mathbb{R}^{d*d}$ is of rank $r$, but we try to recover it using $\mathbf{F} \mathbf{F}^\top$ where $\mathbf{F} \in \mathbb{R}^{d*k}$ and $k>r$, the existing statistical analysis falls short, due to a flat local curvature of the loss function around the global maxima. By decomposing the factorized matrix $\mathbf{F}$ into separate column spaces to capture the effect of extra ranks, we show that $\|\mathbf{F}_t \mathbf{F}_t - \mathbf{X}^*\|_{F}^2$ converges to a statistical error of $\tilde{\mathcal{O}} ({k d \sigma^2/n})$ after $\tilde{\mathcal{O}}(\frac{\sigma_{r}}{\sigma}\sqrt{\frac{n}{d}})$ number of iterations where $\mathbf{F}_t$ is the output of FGD after $t$ iterations, $\sigma^2$ is the variance of the observation noise, $\sigma_{r}$ is the $r$-th largest eigenvalue of $\mathbf{X}^*$, and $n$ is the number of sample. Our results, therefore, offer a comprehensive picture of the statistical and computational complexity of FGD for the over-parameterized matrix sensing problem.

==> 2.formulation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Matrix Sensing Problem}
\label{sec:matrix-sensing-prelim}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\jzcomment{In short, the population update of matrix sensing problem is almost identical to the matrix completion case above}

%\jzcomment{The A matrix here is different from above. Abused the notation a little bit.}
%\subsection{The Matrix Sensing Problem}
Consider the data generating model $y_i = \angles{\matA_i, \trueMat} + \epsilon_i$,
where $\matA_i \in \mathbb{R}^{d*d}$ is the random sensing matrix, $\trueMat \in \mathbb{R}^{d*d}$ is the rank $r$ target matrix we want to recover, and $\epsilon_i$ is a zero-mean sub-Gaussian noise with variance proxy $\sigma^2$. 

We assume that $\trueMat$ is symmetric. The sensing matrix is sampled as follow: each upper triangle entry ($i < j$) $A_{ij}$ is sampled i.i.d. from a zero-mean sub-Gaussian distribution with variance proxy $1$, each lower triangle entry ($i > j$) $A_{ij} = A_{ji}$, and the diagonal entries are sample from i.i.d. from a zero-mean sub-Gaussian distribution with variance proxy $1$.

Given observations $\{ \matA_i, y_i \}_{i=1}^n$, we want to find the optimal $\bX$ subject to a  rank constraint:
\begin{align*}
    \underset{\bX: \bX \succeq 0, \text{rank}(\bX) \leq r}{\arg \min} \frac{1}{4n} \sum_{i=1}^n \left( y_i - \angles{\matA_i, \bX}  \right)^2.
\end{align*}
We can explicitly imposing the rank constraint by reformulating $\bX = \fitMat \fitMat^\top$, where $\fitMat \in \mathbb{R}^{r*d}$, and obtain the following objective:
\begin{align*}
% \label{problem:factored-sensing}
    \underset{\fitMat}{\arg \min} \quad \objFun(\fitMat) := \frac{1}{4n}  \sum_{i=1}^n \left( y_i - \angles{\matA_i, \fitMat \fitMat^T}  \right)^2.
\end{align*}
% If $A_i$ not sym, the sample gradient:
% \begin{align*}
%     \mathbf{G}_t^n = \frac{1}{2n} \sum_{i=1}^n \left( y_i - \angles{\matA_i, \fitMat_t \fitMat_t^{\top}}\right) \left( \matA_i^{\top} + \matA_i   \right)  \fitMat_t.
% \end{align*}
For Problem \ref{formulation:non-convex}, one can solve it directly using gradient descend method with respect to $\fitMat$:
% \begin{align}
% \label{eqn:factored-gradient-method}
%     \fitMat_{t+1} = \fitMat_t - \eta \bG_t^n, \quad \text{where} \quad
%     \mathbf{G}_t^n = \grad \objFun(\fitMat_{t}) = \frac{1}{n} \sum_{i=1}^n \left(  \angles{\matA_i, \fitMat_t \fitMat_t^{\top} - y_i} \right)\matA_i  \fitMat_t,
% \end{align}
where $\eta$ is the step size and $\bG_t^n$ is the gradient evaluated at iteration $t$ with $n$ i.i.d. samples. One can easily check that
$\Exs \left[ \angles{\matA_i, \matB} \matA_i \right] = \matB$
for any matrix $\matB$ with appropriate dimensions.
%\jzcomment{We might also want to study the concentration of this.}
Combined with the fact that $y_i = \angles{\matA_i, \mathbf{X}^*} + \epsilon$,  the population gradient (taking expectation over the observation noise $\epsilon$ and the observation matrices $\matA_i $) is
\begin{align*}
    \mathbf{G}_t := \Exs [ \bG_t^n] = \left(\fitMat_t \fitMat_t^{\top} - \mathbf{X}^* \right)  \fitMat_t.
\end{align*}
% Then the population iteration update is
% \begin{align*}
%     \fitMat_{t+1} = \fitMat_t - \eta \mathbf{G}_t 
%     = \fitMat_{t} - \stepsize \left\lbrace \fitMat_{t} \fitMat_{t}^{\top} \fitMat_{t} - 
%   \mathbf{X}^* \fitMat_{t} \right\rbrace.
% \end{align*}



==> A4.finite_sample_large_T.tex <==

%%%%%%%%%%%%%%%%%%%%=============================%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%=============================%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%=============================%%%%%%%%%%%%%%%%%%%%
\newpage
Now consider the case where $\trueVcoeff$ is not small.

\begin{lemma}
Suppose the sample size $n > C_1 \kappa^2 d \log^3 d \cdot \max(1, \sigma^2/\sigma_r^2)$ for some universal constant $C_1$, and  the step size $\stepsize = \frac{1}{100\sigma_1}$.
Suppose we have good initialization:
\begin{align*}
    \vecnorm{\Ucoeff_0 \Ucoeff_0^T - \trueUcoeff}{2} \leq \rho \sigma_r, \quad
    \vecnorm{\Vcoeff_0 \Vcoeff_0^T - \trueVcoeff}{2} \leq \rho \sigma_r, \quad
    \vecnorm{\Ucoeff_0 \Vcoeff_0^T}{2} \leq \rho \sigma_r, 
    \quad \rm{where } \quad  \rho < 0.1.
\end{align*}
Denote $D_t$ as $\max \{ \vecnorm{\Ucoeff_t \Ucoeff_t^T - \trueUcoeff}{2},  \vecnorm{\Ucoeff_t \Vcoeff_t^T}{2}\}$. Then we have
\begin{align*}
    D_t = A_t + 50 \kappa \sqrt{\frac{d \log d }{n}}\parenth{\sigma + \sigma_r}, \quad \rm{where } \quad  A_{t+1} \leq \parenth{1 - \frac{1}{2} \eta A_t} A_t
\end{align*}
Also,
\begin{align*}
    \vecnorm{\Vcoeff_t \Vcoeff_t^T - \trueVcoeff}{2} \leq 4 \sigma_r
\end{align*}
% \begin{align*}
%     \vecnorm{\Ucoeff_t \Ucoeff_t^T - \trueUcoeff}{2} \leq  C_2 \kappa \sqrt{\frac{d \log d }{n}} \parenth{\frac{1}{t + C_3 \kappa} +  \sigma},\\
%     \vecnorm{\Vcoeff_t \Vcoeff_t^T - \trueVcoeff}{2} \leq C_2 \kappa \sqrt{\frac{d \log d }{n}} \parenth{\frac{1}{t + C_3 \kappa} +  \sigma}, \\
%     \vecnorm{\Ucoeff_t \Vcoeff_t^T}{2} \leq C_2 \kappa \sqrt{\frac{d \log d }{n}} \parenth{\frac{1}{t + C_3 \kappa} +  \sigma}.
% \end{align*}
\end{lemma}
\begin{proof}
\jzcomment{Uniform convergence required.\\}
We prove by induction. 
\jzcomment{Initial condition for the induction.}


We want to further connect $\vecnorm{\Delta_t}{2}$ with $D_t$. Note that with our choice of sample size $n$, according to Lemma \ref{lemma:concentration-Aepsilon} and \ref{lemma:concentration-main} the following holds with probability at least $1 - \exp(- C \log d)$
\begin{align*}
    \vecnorm{\Delta_t}{2} & \leq \sqrt{\frac{d \log d }{n}} \vecnorm{\fitMat_t \fitMat_t^T - \trueMat}{2}+ \sqrt{\frac{d \log d }{n}}\sigma \\
    &\leq \sqrt{\frac{d \log d }{n}} \parenth{\vecnorm{\Ucoeff_t \Ucoeff_t^T - \trueUcoeff}{2} +  \vecnorm{\Vcoeff_t \Vcoeff_t^T - \trueVcoeff}{2} + 2 \vecnorm{\Ucoeff_t \Vcoeff_t^T}{2}}+ \sqrt{\frac{d \log d }{n}}\sigma\\
    &\leq 3\sqrt{\frac{d \log d }{n}} D_t+ \sqrt{\frac{d \log d }{n}}\parenth{\sigma + 4\sigma_r}
\end{align*}
Since $\eta = \frac{1}{100 \sigma_1}$, $\eta \sigma_r = \frac{1}{100 \kappa}$. By choosing $C_1 \geq 1000^2$, and relaxing  $\log d$ to $1$, we have
\begin{align}
\label{eqn:tight-delta_bound-2}
    \vecnorm{\Delta_t}{2} \leq \frac{3}{\sqrt{C_1} \kappa \log d} D_t + \sqrt{\frac{d \log d }{n}}\parenth{\sigma + 4\sigma_r} \leq \frac{3}{10} \eta \sigma_r D_t + \sqrt{\frac{d \log d }{n}}\parenth{\sigma + 4\sigma_r}
\end{align}
We can also obtain a loose bound (not diminishing as $t$ grows) by plugging-in $D_t \leq \rho \sigma_r$ and $n > C_1 \kappa^2 d \log^3 d \cdot \max(1, \sigma^2/\sigma_r^2)$:
\begin{align}
\label{eqn:loose-delta-bound-2}
    \vecnorm{\Delta_t}{2} \leq \frac{6}{\sqrt{C_1} \kappa \log d} \sigma_r \leq \frac{8}{1000} \sigma_r
\end{align}
% By choosing $\log d \sqrt{C_1} \geq 100 C_2$ we can have $\sqrt{\frac{d \log d }{n}} \leq \frac{1}{100 \kappa C_2 }$ and hence by the induction hypothesis we have
% \begin{align}
% \label{eqn:delta_t_upper_bound}
%     \vecnorm{\Delta_t}{2} &\leq \sqrt{\frac{d \log d }{n}} \cdot 4 C_2 \kappa \sqrt{\frac{d \log d }{n}} \parenth{\frac{1}{t + C_3 \kappa} +  \sigma} + \sqrt{\frac{d \log d }{n}}\sigma \\
%     &\leq \frac{1}{25} \sqrt{\frac{d \log d }{n}} \cdot \frac{1}{t + C_3 \kappa} + \frac{26}{25} \sqrt{\frac{d \log d }{n}} \cdot \sigma.
% \end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$\vecnorm{\Ucoeff_t \Ucoeff_t^T - \trueUcoeff}{2}$}
According to \jzcomment{todo} we have
\begin{align*}
    &\vecnorm{\Ucoeff_{t+1}\Ucoeff_{t+1}^T - \trueUcoeff}{2} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(1)}{\leq} & \underbrace{\vecnorm{\mathcal{M}(\Ucoeff_t) \mathcal{M}(\Ucoeff_t)^\top - \trueUcoeff}{2}}_{\text{I}}
    + \underbrace{2\eta \vecnorm{\trueUcoeff}{2} \vecnorm{\Delta_t}{2}}_{\text{V + VIII}}
    + \underbrace{\frac{1}{100}\eta \vecnorm{\Delta_t}{2}^2}_{\text{II}} \\
    & + \underbrace{2\eta \vecnorm{\popUup(\Ucoeff_t)\Ucoeff_t^T - \trueUcoeff}{2} \vecnorm{\Delta_t}{2}}_{\text{III +  VI }}
    + \underbrace{2\eta \vecnorm{\popUup(\Ucoeff_t)\Vcoeff_t^T}{2}\vecnorm{\Delta_t}{2}}_{\text{IV +  VII }}\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(2)}{\leq} & \underbrace{\parenth{1 - \frac{8}{10}\eta\sigma_r } D_t}_{\text{I}} + \underbrace{\frac{1}{50} \vecnorm{\Delta_t}{2}}_{\text{V + VIII}}
    + \underbrace{\frac{1}{100}\eta \vecnorm{\Delta_t}{2}^2}_{\text{II}}
    + \underbrace{4 \eta D_t \vecnorm{\Delta_t}{2}}_{\text{III +  VI + IV +  VII }} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(3)}{\leq} & \underbrace{\parenth{1 - \frac{8}{10}\eta\sigma_r + 4 \eta \parenth{\frac{8}{1000}\sigma_r}} D_t}_{\text{I + III +  VI + IV +  VII}} + \underbrace{\frac{1}{50} \parenth{\frac{3}{10} \eta \sigma_r D_t + \sqrt{\frac{d \log d }{n}}\parenth{\sigma + 4\sigma_r}}}_{\text{V + VIII}} \\
    & + \underbrace{\frac{1}{100}\eta \parenth{\frac{3}{10} \eta \sigma_r D_t + \sqrt{\frac{d \log d }{n}}\parenth{\sigma + 4\sigma_r}} \parenth{\frac{8}{1000}\sigma_r}  }_{\text{II}}\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(4)}{\leq} & \parenth{1 - \frac{8}{10}\eta\sigma_r + \frac{1}{40} \eta \sigma_r + \frac{3}{500}\eta\sigma_r + \frac{8\eta \sigma_r}{100000}  \eta \sigma_r} D_t 
    + \parenth{\frac{1}{50} + \frac{8\eta \sigma_r}{100000}} \sqrt{\frac{d \log d }{n}}\parenth{\sigma +4\sigma_r} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(5)}{\leq} & \parenth{1 - \frac{7}{10}\eta\sigma_r} D_t 
    + \frac{1}{40} \sqrt{\frac{d \log d }{n}}\parenth{\sigma +4\sigma_r}
\end{align*}
where inequality $(2)$ is obtained by the non-expansion property of population update (Equations \ref{eqn:pop_contraction}),  $(3)$ is obtained by plug-in the two relaxation of $\vecnorm{\Delta_t}{2}$ (Equations \ref{eqn:loose-delta-bound-2} and \ref{eqn:tight-delta_bound-2}), $(4)$ is obtained by organizing according to $D_t$ and $\sigma$, and $(5)$ is obtained by $\eta \sigma_r \leq 1/100$. 




\subsection{$\vecnorm{\Ucoeff_t \Vcoeff_t^T }{2}$}
Putting everything above together, we have
\begin{align*}
    &\vecnorm{\Ucoeff_{t+1}\Vcoeff_{t+1}^T }{2} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq & \underbrace{\vecnorm{\popUup(\Ucoeff_t) \popVup(\Vcoeff_t)^\top }{2}}_{\text{I}}
    + \underbrace{\frac{1}{100}\eta \vecnorm{\Delta_t}{2}^2}_{\text{II}}
    + \underbrace{\eta \vecnorm{\popUup(\Ucoeff_t)\Ucoeff_t^T - \trueUcoeff}{2} \vecnorm{\Delta_t}{2} }_{\text{III}} 
    + \underbrace{\eta \vecnorm{\trueUcoeff}{2}\vecnorm{\Delta_t}{2}}_{\text{V }}\\
    & + \underbrace{\eta \vecnorm{\popUup(\Ucoeff_t)\Vcoeff_t^T}{2}\vecnorm{\Delta_t}{2}}_{\text{IV }}
    + \underbrace{\eta \vecnorm{\popVup(\Vcoeff_t)\Ucoeff_t^T}{2}\vecnorm{\Delta_t}{2}}_{\text{VI }}
    + \underbrace{\eta \vecnorm{\popVup(\Vcoeff_t)\Vcoeff_t^T}{2}\vecnorm{\Delta_t}{2}}_{\text{VII }}\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(1)}{\leq} & \underbrace{\parenth{1 - \eta \sigma_r } \vecnorm{\Ucoeff_t \Vcoeff_t^\top}{2} }_{\text{I}}
    + \underbrace{\frac{1}{100}\eta \vecnorm{\Delta_t}{2}^2}_{\text{II}}
    + \underbrace{\eta \vecnorm{\trueUcoeff}{2} \vecnorm{\Delta_t}{2}}_{\text{V}}
    + \underbrace{3 \eta D_t \vecnorm{\Delta_t}{2}}_{\text{III + IV + VI}}
    + \underbrace{3  \eta \sigma_r \vecnorm{\Delta_t}{2}}_{\text{VII}}\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(2)}{\leq} & \underbrace{\parenth{1 - \eta\sigma_r + 3 \eta \parenth{\frac{8}{1000}\sigma_r}} D_t}_{\text{I + III +  VI + IV}} 
    + \underbrace{\frac{1}{100} \parenth{\frac{3}{10} \eta \sigma_r D_t + \sqrt{\frac{d \log d }{n}}\parenth{\sigma + 4\sigma_r}}}_{\text{V}} \\ 
    & + \underbrace{\frac{1}{100}\eta \parenth{\frac{3}{10} \eta \sigma_r D_t + \sqrt{\frac{d \log d }{n}}\parenth{\sigma + 4\sigma_r}} \parenth{\frac{8}{1000}\sigma_r}  }_{\text{II}} \\
    & + \underbrace{3  \eta \sigma_r \parenth{\frac{3}{10} \eta \sigma_r D_t + \sqrt{\frac{d \log d }{n}}\parenth{\sigma + 4\sigma_r}}}_{\text{VII}}\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(3)}{\leq} & \underbrace{\parenth{1 - \eta\sigma_r + 3 \eta \parenth{\frac{8}{1000}\sigma_r}} D_t}_{\text{I + III +  VI + IV}} 
    + \underbrace{\frac{1}{100} \parenth{\frac{3}{10} \eta \sigma_r D_t + \sqrt{\frac{d \log d }{n}}\parenth{\sigma + 4\sigma_r}}}_{\text{V}} \\ 
    & + \underbrace{4  \eta \sigma_r \parenth{\frac{3}{10} \eta \sigma_r D_t + \sqrt{\frac{d \log d }{n}}\parenth{\sigma + 4\sigma_r}}}_{\text{II + VII}}\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(4)}{\leq} & \parenth{1 - \eta\sigma_r + \frac{1}{40} \eta \sigma_r + \frac{3}{500}\eta\sigma_r + \frac{12\eta \sigma_r}{10}  \eta \sigma_r} D_t 
    + \parenth{\frac{1}{100} \sqrt{\frac{d \log d }{n}}
    + 4\eta \sigma_r \sqrt{\frac{d \log d }{n}}}\parenth{\sigma + 4\sigma_r}\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(5)}{\leq} & \parenth{1 - \frac{9}{10}\eta\sigma_r} D_t 
    + \frac{1}{20} \sqrt{\frac{d \log d }{n}}\parenth{\sigma + 4\sigma_r}
\end{align*}
where inequality $(1)$ is obtained by the non-expansion property of population update (Equations \ref{eqn:pop_contraction}),  $(2)$ is obtained by plug-in the two relaxation of $\vecnorm{\Delta_t}{2}$ (Equations \ref{eqn:loose-delta-bound} and \ref{eqn:tight-delta_bound}), $(3)$ is obtained by organizing according to $D_t$ and $\sigma$, and $(4)$ is obtained by $\eta \sigma_r \leq 1/100$. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{$\vecnorm{\Vcoeff_t \Vcoeff_t^T }{2}$}
Following similar deductions as in previous subsections, we have
\begin{align*}
    \Vcoeff_{t+1}\Vcoeff_{t+1}^T 
    = & \underbrace{\popVup(\Vcoeff_t) \popVup(\Vcoeff_t)^T}_{\text{I}}
    + \underbrace{\stepsize^2 \Vmat^T \parenth{ \bG_t -  \bG_t^n}\parenth{ \bG_t -  \bG_t^n}^T \Vmat}_{\text{II}} \\
    & + \stepsize\popVup(\Vcoeff_t)\parenth{ \bG_t -  \bG_t^n}^T \Vmat + \stepsize\Vmat^T \parenth{ \bG_t -  \bG_t^n} \popVup(\Vcoeff_t)^T
\end{align*}
where
\begin{align*}
     \stepsize\popVup(\Vcoeff_t)\parenth{ \bG_t -  \bG_t^n}^T \Vmat 
    = & \underbrace{\stepsize\popVup(\Vcoeff_t)\Ucoeff_t^T \Umat^T \Delta_t \Vmat }_{\text{III}}
    + \underbrace{\stepsize\popVup(\Vcoeff_t)\Vcoeff_t^T \Vmat^T \Delta_t \Vmat}_{\text{IV}}\\
    \stepsize\Vmat^T \parenth{ \bG_t -  \bG_t^n} \popVup(\Vcoeff_t)^T
    = & \underbrace{\stepsize\Vmat^T  \Delta_t \Umat \Ucoeff_t \popVup(\Vcoeff_t)^T}_{\text{V}}
    + \underbrace{\stepsize\Vmat^T  \Delta_t \Vmat \Vcoeff_t \popVup(\Vcoeff_t)^T}_{\text{VI}}
\end{align*}
and
\begin{align*}
    \text{III \& V:}& \quad \quad \quad \vecnorm{\stepsize\popVup(\Vcoeff_t)\Ucoeff_t^T \Umat^T \Delta_t \Vmat}{2} 
    \leq  \eta \vecnorm{\popVup(\Vcoeff_t)\Ucoeff_t^T }{2} \vecnorm{\Delta_t}{2} \\
    \text{IV \& VI:}& \quad \quad \quad \vecnorm{\stepsize\popVup(\Vcoeff_t)\Vcoeff_t^T \Vmat^T \Delta_t \Vmat}{2} 
    \leq \eta \vecnorm{\popVup(\Vcoeff_t)\Vcoeff_t^T}{2}\vecnorm{\Delta_t}{2} \\
    \text{II:}& \quad \quad \quad\vecnorm{\stepsize^2 \Umat^T \parenth{ \bG_t -  \bG_t^n}\parenth{ \bG_t -  \bG_t^n}^T \Umat}{2}  \leq \frac{1}{100}\eta \vecnorm{\Delta_t}{2}^2.
\end{align*}
Note that $\vecnorm{\Vcoeff_{t}\Vcoeff_{t}^T}{2} \leq 3\sigma_r $. Let  $\vecnorm{\Vcoeff_{t}\Vcoeff_{t}^T}{2} = z\sigma_r $ where $z \leq 3$.
\begin{align*}
    &\vecnorm{\Vcoeff_{t+1}\Vcoeff_{t+1}^T}{2} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(1)}{\leq} & \underbrace{\vecnorm{\popVup(\Vcoeff_t) \popVup(\Vcoeff_t)^T}{2}}_{\text{I}}
    + \underbrace{\frac{1}{100}\eta \vecnorm{\Delta_t}{2}^2}_{\text{II}}
    + \underbrace{2\eta \vecnorm{\popVup(\Vcoeff_t)\Ucoeff_t^T }{2} \vecnorm{\Delta_t}{2}}_{\text{III +  V }}
    + \underbrace{2\eta \vecnorm{\popVup(\Vcoeff_t)\Vcoeff_t^T}{2}\vecnorm{\Delta_t}{2}}_{\text{IV +  VI }}\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(2)}{\leq} & \underbrace{\parenth{1 - \eta \vecnorm{\Vcoeff_t \Vcoeff_t^\top}{2} + 2\eta \vecnorm{\trueVcoeff}{2} + 2 \eta   \parenth{\frac{6}{1000}\sigma_r}}z\sigma_r}_{\text{I + IV +  VI}}
    + \underbrace{2\eta D_t \parenth{\frac{6}{1000}\sigma_r} }_{\text{III + V}}
    + \underbrace{\frac{1}{100}\eta \parenth{\frac{6}{1000}\sigma_r}^2 }_{\text{II}} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \overset{(3)}{\leq} &\parenth{1 - \eta z \sigma_r + 2\eta \sigma_r + \frac{12}{1000} \eta   \sigma_r }z\sigma_r + \frac{12}{1000} \eta \sigma_r^2 + \frac{6^2}{100\cdot 1000^2} \eta \sigma_r^2
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % \overset{(4)}{\leq} &\parenth{1 - \eta \vecnorm{\Vcoeff_t \Vcoeff_t^\top}{2} + 3\eta \sigma_r}3\sigma_r \\
\end{align*}
Note that this is quadratic with respect to $z$, and is maximized when $z = \frac{1}{2\eta \sigma_r} + \frac{2012}{2000} > 3$. Plug-in $z = 3$ and we have
\begin{align*}
    \vecnorm{\Vcoeff_{t+1}\Vcoeff_{t+1}^T}{2} &\leq  \parenth{1 - 3 \eta\sigma_r + 2\eta \sigma_r + \frac{12}{1000} \eta   \sigma_r }3\sigma_r + \frac{12}{1000} \eta \sigma_r^2 + \frac{6^2}{100\cdot 1000^2} \eta \sigma_r^2 \\
    &\leq  \parenth{1 - 0.1}3\sigma_r < 3 \sigma_r
\end{align*}
And by triangular inequality,
\begin{align*}
    \vecnorm{\Vcoeff_{t+1}\Vcoeff_{t+1}^T - \trueVcoeff}{2} \leq 4 \sigma_r.
\end{align*}
\end{proof}
